Positivity-preserving discontinuous spectral element methods for compressible multi-species flows

We introduce a novel positivity-preserving, parameter-free numerical stabilisation approach for high-order discontinuous spectral element approximations of compressible multi-species flows. The underlying stabilisation method is the adaptive entropy filtering approach (Dzanic and Witherden, J. Comput. Phys., 468, 2022), which is extended to the conservative formulation of the multi-species flow equations. We show that the straightforward enforcement of entropy constraints in the filter yields poor results around species interfaces and propose an adaptive, parameter-free switch for the entropy bounds based on the convergence properties of the pressure field which drastically improves its performance for multi-species flows. The proposed approach is shown in a variety of numerical experiments applied to the multi-species Euler and Navier--Stokes equations computed on unstructured grids, ranging from shock-fluid interaction problems to three-dimensional viscous flow instabilities. We demonstrate that the approach can retain the high-order accuracy of the underlying numerical scheme even at smooth extrema, ensure the positivity of the species density and pressure in the vicinity of shocks and contact discontinuities, and accurately predict small-scale flow features with minimal numerical dissipation.

==> filter.tex <==
\section{Entropy Filter}
    


\subsection{Pressure Equilibrium}
    \begin{figure}
        \centering
        \adjustbox{width=0.4\linewidth,valign=b}{\input{figs/tikz/pressure_discont.tex}}
        \caption{\label{fig:p_eq_ic}}
    \end{figure}

    To derive the condition on pressure equilibrium we consider the solution shown in \cref{fig:p_eq_ic} for $d=2$. Based on this we would like to show the following:
    \begin{equation}
        \mathbf{1}^T\mathbf{M}\dx{\mathbf{P}}{t} = 0
    \end{equation}
    First consider the conservation of mass equation
    \begin{equation}
        \mathbf{1}^T\mathbf{M}\dx{\pmb{\alpha}_i\pmb{\rho}_i}{t} \approx - \mathbf{1}^T\mathbf{MDF}_{\alpha\rho,i} - \mathbf{1}^T\mathbf{MC}\left[(\mathbf{n}\cdot\mathbf{F}^\mathrm{num}_{\alpha\rho,i}) -\mathbf{N}\hb{L}_\partial\mathbf{F}_{\alpha\rho,i}\right],
    \end{equation}
    applying \cref{eq:c_mat}, and \cref{def:sbp} we obtain
    \begin{equation}
        \mathbf{1}^T\mathbf{M}\dx{\pmb{\alpha}_i\pmb{\rho}_i}{t} \approx -\mathbf{1}^T\mathbf{L}^T_\partial\mathbf{W}_\partial(\mathbf{n}\cdot\mathbf{F}^\mathrm{num}_{\alpha\rho,i}).
    \end{equation}
    Repeating this for the momentum equation we obtain:
    \begin{equation}
        \mathbf{1}^T\mathbf{M}\dx{\pmb{\rho}\mathbf{u}}{t} \approx -\mathbf{1}^T\mathbf{L}^T_\partial\mathbf{W}_\partial(\mathbf{n}\cdot\mathbf{F}^\mathrm{num}_{\rho u}).
    \end{equation}
    Therefore, to achieve a constant velocity condition we require that $\dxvar{\rho u}{t} = u\sum_i\dxvar{\alpha_i\rho_i}{t}$, which leads to the  condition at a flux point $j$ that
    \begin{equation}
        (\mathbf{n}\cdot\mathbf{F}_{\rho u}^\mathrm{num})_j = u_j\sum_i(\mathbf{n}\cdot\mathbf{F}_{\alpha\rho,i}^\mathrm{num})
    \end{equation}


==> notes.tex <==
\section{Flux Reconstruction}\label{sec:fr}

\begin{equation}
    \dx{\mathbf{u}}t \approx - \mathbf{DF} - \mathbf{C}\left[(\mathbf{n}\cdot\mathbf{F}^\mathrm{num}) - \mathbf{N}\hb{L}_\partial\mathbf{F} \right]
\end{equation}

\begin{definition}[Summation-by-parts]\label{def:sbp}
  For solutions $u\in C^1(K)$ and $U\in (C^1(K))^d$, let  $u_i$ and $U_i$ be approximations in element $K_i$ such that for some nodal point set $\mathbf{x}_i\{\mathbf{x}_{i,j}\}_{j\leq N_s}$ we have $\mathbf{u}_i = u_i(\mathbf{x}_i)$ and $\mathbf{U}_i = U_i(\mathbf{x}_i)$, then a set of operators is said to satisfy the generalised \ac{sbp} property if:
  \begin{equation}\label{eq:sbp}
    \mathbf{MD} + \mathbf{G}^T\hb{M} = \mathbf{L}^T_{\partial K}\mathbf{W}_{\partial K}\mathbf{N}\hb{L}_{\partial K},
  \end{equation}
  where the divergence and gradient operators are defined as
  \begin{equation}
  \mathbf{DU}_i = [\mathbf{D}_{x_1}, \mathbf{D}_{x_2}, \dots]\mathbf{U}_i = \nabla\cdot U_i \quad \mathrm{and} \quad \mathbf{Gu}_i = 
  \begin{bmatrix}
    \mathbf{D}_{x_1}\\ \mathbf{D}_{x_2}\\\vdots
  \end{bmatrix}\mathbf{u} = \nabla u_i.
  \end{equation}
        Then defining the interpolation operator $\mathbf{L}_{\partial K}:K\mapsto\partial K$, and surface mass matrix, $\mathbf{W}_{\partial K}$, such that
        \begin{equation}
            \mathbf{u}_i^T\mathbf{L}_{\partial K}\mathbf{W}_{\partial K}\mathbf{N}\hb{L}_{\partial K}\mathbf{U}_i = \int_{\partial K}u_iU_i\cdot \mathbf{n}_i\mathrm{d}s,
        \end{equation}
  where $\mathbf{n}$ is a vector of outwards facing normals at the interface. Finally, the Kronecker product of a matrix with the identity matrix is denoted by
  \begin{equation}
    \hb{A} = \mathbf{I}_d\otimes\mathbf{A}.
  \end{equation}
\end{definition}

Then from \citep{Ranocha2016,Trojak2023}, \ac{fr} is linearly stable and conservative when
\begin{equation}\label{eq:c_mat}
  \mathbf{C} = (\mathbf{M} + \mathbf{Q})^{-1}\mathbf{L}_\partial^T\mathbf{W}_\partial,
\end{equation}
subject to conditions on $\mathbf{Q}$. In this work we will restrict $\mathbf{Q}=\mathbf{0}$ for brevity.

///// Just some notes on the pressure derivative:
    \begin{equation}
        \px{P}{t} = (\gamma-1)\left[\px{E}{t} - P\px{}{t}\left(\frac{1}{\gamma-1}\right) - \half u^2\px{\rho}{t}\right]
    \end{equation}
    For $n=2$
    \begin{equation}
        \px{}{t}\left(\frac{1}{\gamma-1}\right) = \left[\frac{c_{p,1}c_{v,0} - c_{p,0}c_{v,1}}{(c_{p,0} - c_{v,0})\alpha_0\rho_0 + (c_{p,1} - c_{v,1})\alpha_1\rho_1}\right]\left(\alpha_1\rho_1\px{\alpha_0\rho_0}{t} - \alpha_0\rho_0\px{\alpha_1\rho_1}{t}\right)
    \end{equation}


    // Tarik's scratch
    \begin{equation}
        P = (\gamma - 1) \left[E - \half \frac{\rho u^2}{\rho} \right]
    \end{equation}
    \begin{equation}
        \partial_t P = \frac{P}{\gamma -1} \partial_t (\gamma - 1)  + (\gamma - 1) \left [\partial_t E - \half \partial_t \frac{\rho u^2}{\rho} \right]
    \end{equation}
    \begin{equation}
        \partial_x P = \partial_x u = 0
    \end{equation}
    \begin{equation}
        \partial_t \rho = -\partial_x \rho u = -u \partial_x \rho
    \end{equation}
    \begin{equation}
        \partial_t \rho u = -\partial_x (\rho u^2  + P)= -u \partial_x \rho u
    \end{equation}
    \begin{equation}
        \partial_t E = -\partial_x (uE  + uP)= -u \partial_x E = -u \partial_x \left (\frac{P}{\gamma -1} + \half \frac{\rho u^2}{\rho} \right) = u \frac{P}{\gamma-1} \frac{\partial_x (\gamma -1)}{\gamma-1} - \half u \partial_x \left (\frac{\rho u^2}{\rho} \right)
    \end{equation}
    \begin{equation}
        \partial_t \left(\frac{\rho u^2}{\rho} \right) = 2 \frac{\rho u}{\rho} \partial_t \rho u - 2 \frac{\rho u^2}{\rho^2} \partial_t \rho = - 2 u \partial_x \rho u \left (\frac{\rho u}{\rho} \right) + 2 u \partial_x \rho \left (\frac{\rho u^2}{\rho^2} \right) = -2u^2 \partial_x \rho u + 2 u^3 \partial_x \rho = 0
    \end{equation}
    \begin{equation}
        \gamma - 1 = \frac{\alpha_0\rho_0 c_{p, 0} + \alpha_1\rho_1 c_{p, 1}}{\alpha_0\rho_0 c_{v, 0} + \alpha_1\rho_1 c_{v, 1}} - 1
    \end{equation}
    \begin{equation}
        \partial_t (\gamma - 1) = (c_{p, 1}c_{v, 0} - c_{p, 0}c_{v, 1})\frac{\alpha_0\rho_0 \partial_t \alpha_1\rho_1 - \alpha_1\rho_1 \partial_t \alpha_0\rho_0}{(\alpha_0\rho_0 c_{v, 0} + \alpha_1\rho_1 c_{v, 1})^2} = -u (c_{p, 1}c_{v, 0} - c_{p, 0}c_{v, 1})\frac{\alpha_0\rho_0 \partial_x \alpha_1\rho_1 - \alpha_1\rho_1 \partial_x \alpha_0\rho_0}{(\alpha_0\rho_0 c_{v, 0} + \alpha_1\rho_1 c_{v, 1})^2}
    \end{equation}
    \begin{equation}
        \partial_x (\gamma - 1) = (c_{p, 1}c_{v, 0} - c_{p, 0}c_{v, 1})\frac{\alpha_0\rho_0 \partial_x \alpha_1\rho_1 - \alpha_1\rho_1 \partial_x \alpha_0\rho_0}{(\alpha_0\rho_0 c_{v, 0} + \alpha_1\rho_1 c_{v, 1})^2}
    \end{equation}
    \begin{equation}
        \partial_t (\gamma - 1) = -u \partial_x (\gamma - 1)
    \end{equation}
    \begin{equation}
        \partial_t P = \frac{P}{\gamma -1} \partial_t (\gamma - 1)  + (\gamma - 1) \partial_t E = -u \frac{P}{\gamma-1} \partial_x (\gamma -1) + u \frac{P}{\gamma-1} \partial_x (\gamma -1) - \half u \partial_x \left (\frac{\rho u^2}{\rho} \right)
    \end{equation}
    

    //// Some more notes on entropy and pressure equilibrium.
    From the first and second law we have
    \begin{equation}
        T\mathrm{d}\sigma = \mathrm{h} - v\mathrm{p}
    \end{equation}
    with 
    \begin{equation}
        c_v = \px{e}{T}\bigg|_v, \quad \mathrm{and} \quad c_p = \px{h}{T}\bigg|_P.
    \end{equation}
    Assuming an ideal gas we have
    \begin{equation}
        \mathrm{d}\sigma = \frac{c_p(T)}{T}\mathrm{d}T - \frac{R}{P}\mathrm{d}P
    \end{equation}
    Further assuming $c_p$ and $c_v$ are constant ie $e=c_vT$ and $h=c_pT$, then we have
    \begin{equation}
        \mathrm{d}\sigma = \frac{c_p}{e}\mathrm{d}e - \frac{R}{P}\mathrm{d}P
    \end{equation}
    Therefore we form the transport equation
    \begin{equation}\label{eq:s_mat}
        \px{\sigma}{t} + u\px{\sigma}{x} = \frac{c_p}{e}\left(\px{e}{t} + u\px{e}{x}\right) - \frac{R}{P}\left(\px{P}{t} + u\px{P}{x}\right) = 0,
    \end{equation}
    where the equality comes from the transport of entropy, see Eq. (2.3) in \citet{Gouasmi2020}. For the interface we also have that
    \begin{equation}
        \px{e}{t} + u\px{e}{x} = -\frac{P}{\rho}\px{u}{x},
    \end{equation}
    substituting this into \cref{eq:s_mat} we obtain
    \begin{equation}
        -\frac{c_pP}{\rho e}\px{u}{x} - \frac{R}{P}\left(\px{P}{t} + u\px{P}{x}\right) = 0.
    \end{equation}
    Using $R = c_p - c_v$ and $P=(\gamma-1)\rho e$
    \begin{equation}
        \px{P}{t} + u\px{P}{x} = -\gamma P\px{u}{x}.
    \end{equation}
    

==> tikz/temp.tex <==
% do not delete

